Pan-tumor CAnine cuTaneous Cancer Histology (CATCH) dataset

Due to morphological similarities, the differentiation of histologic sections of cutaneous tumors into individual subtypes can be challenging. Recently, deep learning-based approaches have proven their potential for supporting pathologists in this regard. However, many of these supervised algorithms require a large amount of annotated data for robust development. We present a publicly available dataset of 350 whole slide images of seven different canine cutaneous tumors complemented by 12,424 polygon annotations for 13 histologic classes, including seven cutaneous tumor subtypes. In inter-rater experiments, we show a high consistency of the provided labels, especially for tumor annotations. We further validate the dataset by training a deep neural network for the task of tissue segmentation and tumor subtype classification. We achieve a class-averaged Jaccard coefficient of 0.7047, and 0.9044 for tumor in particular. For classification, we achieve a slide-level accuracy of 0.9857. Since canine cutaneous tumors possess various histologic homologies to human tumors the added value of this dataset is not limited to veterinary pathology but extends to more general fields of application.

==> arxiv_ Pan-Tumor Whole Slide Image Dataset for Canine Cutaneous Tumor Segmentation and Classification/tables/annotations.tex <==
\begin{table}[H]
\centering
\begin{tabular}{|lS[table-format = 5.0]S[table-format = 5.2]|}
\hline
Class & \multicolumn{1}{l}{Annotation Polygons} & \multicolumn{1}{l|}{Annotation Area [\si{\milli\meter^2}]} \\
\hline
epidermis & 3188 & 2244.57 \\
dermis & 3423 & 16561.82  \\
subcutis & 2850 & 7367.62 \\
bone & 51 & 216.86 \\
cartilage & 16 & 32.15 \\
inflammation \& necrosis & 719 & 2048.54 \\
melanoma & 379 & 6836.61 \\
histiocytoma & 369 & 2941.12 \\
plasmacytoma & 377 & 4750.31 \\
trichoblastoma & 423 & 9072.10 \\
\acl{mct} & 161 & 9329.85 \\
\acl{scc} & 337 & 3513.56 \\
\acl{pnst} & 131 & 11108.78 \\
\hline
total & 12424 & 76023.89 \\
\hline
\end{tabular}
\caption{\label{tab:annotations}Annotated polygons and area per tissue class.}
\end{table}

==> arxiv_ Pan-Tumor Whole Slide Image Dataset for Canine Cutaneous Tumor Segmentation and Classification/tables/datasets.tex <==
\begin{table}[H]
\centering
\begin{adjustbox}
{ width=\textwidth}
\begin{tabular}{|lllS[table-format = 5.0]lS[table-format = 2.0]ll|}
\hline
Dataset  & Year & Organ & \multicolumn{1}{l}{Images} & Image Type & \multicolumn{1}{l}{Classes} & Class Details &  \multicolumn{1}{l|}{Annotation Type}  \\
\hline
CAMELYON16 \cite{litjens2018} & 2016 & breast & 399 & \aclp{wsi} & 2 & tumor types & contours \\
CAMELYON17 \cite{litjens2018} & 2017 & breast & 1000 & \aclp{wsi}  & 5 & tumor stagings & image-level (all images)\\  
& & & & & 3 & tumor types &  contours (50 images) \\
\acs{bach} \cite{aresta2019} & 2018 & breast & 500 & patches & 4 & tumor types & image-level \\ 
 & & & 40 & \aclp{wsi} &  4 & tumor types & contours (10 images)\\ 
\acs{paip} \cite{kim2021} & 2019 & liver & 100 & \aclp{wsi} & 2 & whole tumor + viable tumor & contours \\
\acs{adp} \cite{hosseini2019} & 2019 & multi-organ & 17668 & patches & 57 & benign tissues & image-level \\ 
\acs{bracs} \cite{pati2022} & 2021 & breast & 4537 & patches & 7 & tumor types & image-level\\ 
& & breast & 574 & \aclp{wsi} & 7 & tumor types & image-level\\ 
\acs{droid} \cite{stadler2021} & 2021 & ovarian & 193 & \aclp{wsi} & 11 & ovarian tissue + tumor types & contours\\
& & breast & 361 & \aclp{wsi} & 4 & tumor types & contours\\
& & skin  & 99 & \aclp{wsi} & 32 &  benign + abnormal tissues & contours\\
& & colon  & 101 & \aclp{wsi} & 38 & benign + abnormal tissues & contours\\
\acs{catch} (ours) & 2022 & skin & 350 & \aclp{wsi} & 13 & skin tissue + tumor types & contours\\ 
\hline
\end{tabular}
\end{adjustbox}
\caption{\label{tab:datasets}Publicly available datasets for segmentation tasks on histological specimens.}
\end{table}

==> arxiv_ Pan-Tumor Whole Slide Image Dataset for Canine Cutaneous Tumor Segmentation and Classification/tables/generalized_ci.tex <==
\begin{table}[H]
\centering
\begin{tabular}{|lS[table-format = 1.4]S[table-format = 1.4]S[table-format = 1.4]S[table-format = 1.4]S[table-format = 1.4]|}
\hline
Class & \multicolumn{1}{l}{$CI_{r1, r2}$} & \multicolumn{1}{l}{$CI_{r1, r3}$} & \multicolumn{1}{l}{$CI_{r2, r3}$}&
\multicolumn{1}{l}{$CI_{pairs}$}&
\multicolumn{1}{l|}{$CI_{gen}$} \\
\hline
background & 0.9130 & 0.9239 & 0.9319 & 0.9229 & 0.9229 \\
tumor & 0.8501 & 0.8506 & 0.8535 & 0.8514 & 0.8514 \\
epidermis & 0.8025 & 0.7228 & 0.7270 & 0.7508 & 0.7512 \\
dermis & 0.6875 & 0.7015 & 0.7659 & 0.7183 & 0.7169 \\
subcutis & 0.5254 & 0.5872 & 0.6421 & 0.5849 & 0.5836 \\
inflammation \& necrosis & 0.2823 & 0.3040 & 0.3895 & 0.3253 & 0.3302 \\
\hline
\end{tabular}
\caption{\label{tab:gci}Class-wise conformity index computed for all unique pairs of annotators. $CI_{pairs}$ averages the pair-wise conformity indices whereas $CI_{gen}$ is a generalized version of the Jaccard coefficient.}
\end{table}

				
				
				


==> arxiv_ Pan-Tumor Whole Slide Image Dataset for Canine Cutaneous Tumor Segmentation and Classification/tables/iou.tex <==

\begin{table}[H]
\centering
\begin{tabular}{|lS[table-format = 1.4]S[table-format = 1.4]S[table-format = 1.4]S[table-format = 1.4]|}
\hline
Class & \multicolumn{1}{l}{\ac{wsi}} & \multicolumn{1}{l}{\ac{roi}$_{r1}$} & \multicolumn{1}{l}{\ac{roi}$_{r2}$}  & \multicolumn{1}{l|}{\ac{roi}$_{r3}$ }  \\
\hline
background & 0.9757 & 0.9362 & 0.9355 & 0.9430 \\
tumor & 0.9044 & 0.8399 & 0.7911 & 0.8193 \\
epidermis & 0.6661 & 0.7033 & 0.6685 & 0.6167 \\
dermis & 0.6753 & 0.6988 & 0.6285 & 0.6740 \\
subcutis & 0.7043 & 0.6232 & 0.5101 & 0.6435 \\
inflammation \& necrosis & 0.3023 & 0.2816 & 0.1331 & 0.1646 \\
\hline
\end{tabular}
\caption{\label{tab:jaccard}Class-wise Jaccard similarity score for all \acp{wsi} of the test set annotated by rater 1 and the \aclp{roi} evaluated in the inter-rater experiments annotated by raters 1, 2, and 3.}
\end{table}

==> arxiv_ Pan-Tumor Whole Slide Image Dataset for Canine Cutaneous Tumor Segmentation and Classification/tables/iou_subtypes.tex <==
\begin{table}[H]
\centering
\begin{tabular}{|lS[table-format = 1.4]|}
\hline
Class & \multicolumn{1}{l|}{Tumor \ac{wsi} Jaccard Score} \\
\hline
melanoma & 0.8394\\
histiocytoma & 0.8714\\
plasmacytoma & 0.9419\\
trichoblastoma & 0.9650\\
\acl{mct} & 0.8721\\
\acl{scc} & 0.7185\\
\acl{pnst} & 0.9166\\
\hline
\end{tabular}
\caption{\label{tab:jaccard_sub_type}Tumor Jaccard similarity score computed from the confusion matrix accumulated over all ten test \acp{wsi} of the respective subtype.}
\end{table}

==> arxiv_ Pan-Tumor Whole Slide Image Dataset for Canine Cutaneous Tumor Segmentation and Classification/tables/metrics.tex <==
\begin{table}[H]
\centering
\begin{tabular}{|lS[table-format = 1.4]S[table-format = 1.4]S[table-format = 1.4]|}
\hline
Class & \multicolumn{1}{l}{Precision} & \multicolumn{1}{l}{Recall} & \multicolumn{1}{l|}{F$_1$~score}\\
\hline
melanoma & 0.8555 & 0.9675 & 0.9081\\
histiocytoma & 0.9399 & 0.9679 & 0.9537\\
plasmacytoma & 0.9684 & 0.9624 & 0.9654\\
trichoblastoma & 0.9478 & 0.9568 & 0.9522\\
\acl{mct} & 0.9886 & 0.9584 & 0.9732\\
\acl{scc} & 0.8251 & 0.9367 & 0.8773\\
\acl{pnst} & 0.9783 & 0.9182 & 0.9473\\
\hline
\end{tabular}
\caption{\label{tab:metrics}Patch-level tumor precision, recall and F$_1$~score per tumor subtype.}
\end{table}
